HORAE: A Domain-Agnostic Language for Automated Service Regulation

Artificial intelligence is rapidly encroaching on the field of service regulation. However, existing AI-based regulation techniques are often tailored to specific application domains and thus are difficult to generalize in an automated manner. This paper presents Horae, a unified specification language for modeling (multimodal) regulation rules across a diverse set of domains. We showcase how Horae facilitates an intelligent service regulation pipeline by further exploiting a fine-tuned large language model named RuleGPT that automates the Horae modeling process, thereby yielding an end-to-end framework for fully automated intelligent service regulation. The feasibility and effectiveness of our framework are demonstrated over a benchmark of various real-world regulation domains. In particular, we show that our open-sourced, fine-tuned RuleGPT with 7B parameters suffices to outperform GPT-3.5 and perform on par with GPT-4o.

==> macros.tex <==
% !TEX root = ./main.tex
%
\RequirePackage{todonotes}

% TODOS
%\setlength{\marginparwidth}{1.5cm}

\newcommand{\cmscomment}[1]{\todo[color=blue!10,size=\small,fancyline,author=CMS]{#1}\xspace}
\newcommand{\cmscommentinline}[1]{\todo[inline,color=blue!10,author=CMS]{#1}\xspace}
\newcommand{\atcms}{\colorbox{blue!10}{\textbf{@CMS}}}

\newcommand{\sytcomment}[1]{\todo[color=green!10,size=\small,fancyline,author=SYT]{#1}\xspace}
\newcommand{\sytcommentinline}[1]{\todo[inline,color=green!10,author=SYT]{#1}\xspace}
\newcommand{\atsyt}{\colorbox{green!10}{\textbf{@SYT}}}

\newcommand{\cjtcomment}[1]{\todo[color=green!25,size=\small,fancyline,author=CJT]{#1}\xspace}
\newcommand{\cjtcommentinline}[1]{\todo[inline,color=green!25,author=CJT]{#1}\xspace}
\newcommand{\atcjt}{\colorbox{green!25}{\textbf{@CJT}}}

\newcommand{\zkjcomment}[1]{\todo[color=cyan!30,size=\small,fancyline,author=ZKJ]{#1}\xspace}
\newcommand{\zkjcommentinline}[1]{\todo[inline,color=cyan!30,author=ZKJ]{#1}\xspace}
\newcommand{\atzkj}{\colorbox{cyan!30}{\textbf{@ZKJ}}}

\newcommand{\lhcomment}[1]{\todo[color=orange!25,size=\small,fancyline,author=LH]{#1}\xspace}
\newcommand{\lhcommentinline}[1]{\todo[inline,color=orange!25,author=LH]{#1}\xspace}
\newcommand{\atlh}{\colorbox{orange!25}{\textbf{@LH}}}

\newcommand{\ztccomment}[1]{\todo[color=blue!25,size=\small,fancyline,author=ZTC]{#1}\xspace}
\newcommand{\ztccommentinline}[1]{\todo[inline,color=blue!25,author=ZTC]{#1}\xspace}
\newcommand{\atztc}{\colorbox{blue!25}{\textbf{@ZTC}}}

\newcommand{\wzycomment}[1]{\todo[color=blue!25,size=\small,fancyline,author=WZY]{#1}\xspace}
\newcommand{\wzycommentinline}[1]{\todo[inline,color=blue!25,author=WZY]{#1}\xspace}
\newcommand{\atwzy}{\colorbox{blue!25}{\textbf{@WZY}}}

\newcommand{\ylycomment}[1]{\todo[color=orange!25,size=\small,fancyline,author=YLY]{#1}\xspace}
\newcommand{\ylycommentinline}[1]{\todo[inline,color=orange!25,author=YLY]{#1}\xspace}
\newcommand{\atyly}{\colorbox{orange!25}{\textbf{@YLY}}}

\newcommand{\rvcomment}[1]{\todo[color=red!10,size=\small,fancyline,author=Reviewer]{#1}\xspace}

\newcommand{\sfsymbol}[1]{\textsf{\upshape {#1}}}
\newcommand{\boldsfsymbol}[1]{\textbf{\textsf{\upshape {#1}}}}
\newcommand{\ttsymbol}[1]{\texttt{\upshape {#1}}}

%colors
\newcommand{\green}[1]{\textcolor{ForestGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\nblue}[1]{\textcolor{NavyBlue}{#1}}
\newcommand{\red}[1]{\textcolor{Red}{#1}}
\newcommand{\orange}[1]{\textcolor{RedOrange}{#1}}
\newcommand{\gray}[1]{\textcolor{Gray}{#1}}
\newcommand{\maroon}[1]{\textcolor{Maroon}{#1}}
\newcommand{\violet}[1]{\textcolor{Violet}{#1}}

\definecolor{111}{HTML}{2E75B6}
\definecolor{222}{HTML}{ED7D31}
\definecolor{333}{HTML}{A2175F}
\definecolor{444}{HTML}{385723}
\definecolor{555}{HTML}{7C7C7C}
\definecolor{666}{HTML}{176D55}

%revision
\newcommand{\rev}[1]{\blue{#1}}
\newcommand{\add}[1]{\blue{#1}}
% \newcommand\remove{\bgroup\markoverwith{\red{\rule[.4ex]{2pt}{1pt}}}\ULon}
\newcommand\remove[1]{\red{#1}}
% \newcommand\remove[1]{}
% \newcommand\removedisplay{\bgroup\markoverwith{\red{\rule[1ex]{2pt}{1pt}}}\ULon}
% \everydisplay{\let\remove\removedisplay}
\newcommand{\change}[2]{\remove{#1}\add{#2}}

%marks
\newcommand{\cmark}{\textcolor{ForestGreen}{\ding{51}}}%
\newcommand{\xmark}{\textcolor{Maroon}{\ding{55}}}%
\newcommand{\namark}{\textcolor{Maroon}{\textbf{?}}}%

\newcommand{\Cmark}{\textcolor{ForestGreen}{\Large\ding{51}}}%
\newcommand{\Xmark}{\textcolor{Maroon}{\Large\ding{55}}}%
\newcommand{\NAmark}{\textcolor{Maroon}{\Large\textbf{?}}}%


% Math
\newcommand{\Nats}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\NatsInf}{\mathbb{N}^\infty\xspace}
\newcommand{\PosNats}{\ensuremath{\mathbb{N}_{>0}}\xspace}
\newcommand{\Ints}{\ensuremath{\mathbb{Z}}\xspace}
\newcommand{\Rats}{\ensuremath{\mathbb{Q}}\xspace}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\StrictPosReals}{\mathbb{R}_{> 0}}
\newcommand{\PosReals}{\mathbb{R}_{\geq 0}}
\newcommand{\PosRats}{\mathbb{Q}_{\geq 0}}
\newcommand{\PosRealsInf}{\mathbb{R}_{\geq 0}^\infty}

\newcommand{\RR}{\Reals}
\newcommand{\NN}{\Nats}
\newcommand{\BB}{\ensuremath{\mathbb{B}}\xspace}

\newcommand{\prob}{\ensuremath{\mathbb{P}}\xspace}
\newcommand{\measure}{\ensuremath{\textit{Pr}}\xspace}

\newcommand{\EE}{\mathit{E}}
\newcommand{\FF}{\mathbb{E}}
\newcommand{\Expectations}{\FF}
\renewcommand{\SS}{\mathbb{S}}
%\newcommand{\PP}{\mathbb{P}}

\newcommand{\TRUE}{\ensuremath{\mathsf{true}}}
\newcommand{\FALSE}{\ensuremath{\mathsf{false}}}

\newcommand{\TT}{\ensuremath{\mathcal{T}}}
\newcommand{\interp}{\ensuremath{I}}
\newcommand{\interps}{\ensuremath{\mathcal{I}}}

\newcommand{\precision}{\ensuremath{\mathcal{P}}}
\newcommand{\recall}{\ensuremath{\mathcal{R}}}
\newcommand{\fscore}{\ensuremath{\mathcal{F}_1}}

\newcommand{\interpQT}{\ensuremath{I_{\scriptscriptstyle\#}}}
\newcommand{\interpsQT}{\ensuremath{\mathcal{I}_{\scriptscriptstyle\#}}}

\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\newcommand{\primed}[1]{\ensuremath{{#1}^{\prime}}}

%% rotated R
\newcommand{\rotR}{\rotatebox[origin=c]{180}{R}}

%for qedT mark compatible within displaymath
\def\triangleforqed{\hbox{$\lhd$}}
\makeatletter
\DeclareRobustCommand{\qedT}{%
	\ifmmode
	\eqno \def\@badmath{$$}%$$
	\let\eqno\relax \let\leqno\relax \let\veqno\relax
	\hbox{\triangleforqed}%
	\else
	\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
	\quad\hbox{\triangleforqed}%
	\fi
}
\makeatother

%%Languages
%\font\tt=rm-lmtl10
%\font\btt=rm-lmtk10
%%\newcommand{\code}[1]{{\fontfamily{cmtt}\fontseries{m}\fontshape{n}\selectfont\small{#1}}}
%\newcommand{\code}[1]{{\fontfamily{cmtt}\fontseries{m}\fontshape{n}\selectfont#1}}
%%\newcommand{\codeBold}[1]{{\ttfamily\fontseries{b}\fontshape{n}\selectfont#1}}
%\newcommand{\codeBold}[1]{#1}
\newcommand{\langname}{\textsc{Horae}\xspace}
\newcommand{\langnameNaked}{Horae\xspace}
\newcommand{\gptname}{\textnormal{RuleGPT}\xspace}
\newcommand{\gptnameNaked}{RuleGPT\xspace}
\newcommand{\datasetname}{\text{SRR-Eval}\xspace}
\newcommand{\datasetnameNaked}{SRR-Eval\xspace}
\newcommand{\codify}[1]{\textup{\texttt{#1}}}
\newcommand{\pgcl}{\codify{pGCL}\xspace}
\newcommand{\gcl}{\codify{GCL}\xspace}

%vphantom is used to vertically align underbraces
\newcommand{\rulefont}[1]{\mathsf{#1}\vphantom{y}}
\newcommand{\rulefontColor}[1]{\textcolor{NavyBlue}{\mathsf{#1}\vphantom{y}}}

\newcommand{\jstring}[1]{\texttt{"}#1\texttt{"}}

\newcommand{\type}{\ensuremath{\mathtt{type}}\xspace}
\newcommand{\stmt}{\ensuremath{s}\xspace}
\newcommand{\timestamp}{\ensuremath{\textcolor{RedOrange}{\tau}}\xspace}
\newcommand{\timestampPlain}{\ensuremath{\tau}\xspace}
\newcommand{\event}{\ensuremath{\textcolor{NavyBlue}{e}}\xspace}
\newcommand{\eventPlain}{\ensuremath{e}\xspace}

\newcommand{\key}[1]{\ensuremath{\textcolor{ForestGreen}{\mathsf{#1}}}\xspace}
\newcommand{\shall}{\key{shall}}
\newcommand{\should}{\key{should}}
\newcommand{\forbid}{\key{forbid}}

%\newcommand{\lneg}{\textcolor{ForestGreen}{\neg}\xspace}
%\newcommand{\lwedge}{\xspace\textcolor{ForestGreen}{\wedge}\xspace}
%\newcommand{\lvee}{\xspace\textcolor{ForestGreen}{\vee}\xspace}

\newcommand{\component}[1]{\ensuremath{\textit{#1}}\xspace}
\newcommand{\obj}{\component{object}}
\newcommand{\act}{\component{action}}
\newcommand{\attr}{\component{attribute}}
\newcommand{\val}{\component{value}}
\newcommand{\adj}{\component{adjective}}

\newcommand{\rulelib}{\ensuremath{\textit{RLib}}\xspace}
\newcommand{\semQL}[1]{\left\llbracket #1 \right\rrbracket}
\newcommand{\semQT}[1]{\left\llbracket #1 \right\rrbracket_{\scriptscriptstyle\#}}


%%%%    Standards    %%%%

\newcommand{\mydot}{\text{{\large\textbf{.}}\,}}
\DeclareMathOperator{\dif}{\,d\!}
\newcommand{\TAG}[1]{{\tag{\small{{#1}}}}}

%%%%    Shortcuts    %%%%

\newcommand{\tiff}{\textnormal{iff}\quad}
\newcommand{\qiff}{\ \quad\textnormal{iff}\quad\ }
\newcommand{\qqiff}{\qquad\textnormal{iff}\qquad}
\newcommand{\lqiff}{\textnormal{iff}\quad}
\newcommand{\lqqiff}{\textnormal{iff}\qquad}

\newcommand{\aand}{\ \ \textnormal{and}\ \ }
\newcommand{\qand}{\ \quad\textnormal{and}\quad\ }
\newcommand{\qqand}{\qquad\textnormal{and}\qquad}

\newcommand{\oor}{\ \ \textnormal{or}\ \ }
\newcommand{\qor}{\ \quad\textnormal{or}\quad\ }
\newcommand{\qqor}{\qquad\textnormal{or}\qquad}

\newcommand{\wwith}{\ \ \textnormal{with}\ \ }
\newcommand{\qwith}{\ \quad\textnormal{with}\quad\ }
\newcommand{\qqwith}{\qquad\textnormal{with}\qquad}

\newcommand{\qimplies}{\ \quad\textnormal{implies}\quad\ }
\newcommand{\qqimplies}{\qquad\textnormal{implies}\qquad}
\newcommand{\lqimplies}{\textnormal{implies}\quad}
\newcommand{\lqqimplies}{\textnormal{implies}\qquad}

\newcommand{\pprec}{\mathrel{{\prec}\hspace{-.5ex}{\prec}}}
\newcommand{\ppprec}{~{}\pprec{}~}
\newcommand{\npprec}{\centernot\pprec}


\newcommand{\ppreceq}{~{}\preceq{}~}
\newcommand{\ssucceq}{~{}\succeq{}~}
\newcommand{\defeq}{{}\triangleq{}}
\newcommand{\ddefeq}{\ {}\defeq{}\ }
\newcommand{\eeq}{~{}={}~}
\newcommand{\mmapsto}{~{}\mapsto{}~}
\newcommand{\eequiv}{~{}\equiv{}~}
\newcommand{\pplus}{~{}+{}~}
\newcommand{\ccdot}{~{}\cdot{}~}
\newcommand{\llongrightarrow}{~{}\longrightarrow{}~}
\newcommand{\qlongrightarrow}{\quad{}\longrightarrow{}\quad}
\newcommand{\qqlongrightarrow}{\qquad{}\longrightarrow{}\qquad}
\newcommand{\mmid}{~{}\mid{}~}
\newcommand{\qmid}{\quad{}|{}\quad}
\newcommand{\tto}{~{}\to{}~}
\newcommand{\uuplus}{\,{}\uplus{}\,}
\newcommand{\nneq}{~{}\neq{}~}
\newcommand{\qeq}{\quad{}={}\quad}
\newcommand{\qqeq}{\qquad{}={}\qquad}
\newcommand{\lleq}{~{}\leq{}~}
\newcommand{\LL}{~{}<{}~}
\newcommand{\GG}{~{}>{}~}
\newcommand{\ggeq}{~{}\geq{}~}
\newcommand{\ssqsubseteq}{~{}\sqsubseteq{}~}
\newcommand{\iimplies}{~{}\implies{}~}
\newcommand{\mmodels}{~{}\models{}~}
\newcommand{\nnotmodels}{~{}\not\models{}~}
\newcommand{\iin}{~{}\in{}~}
\newcommand{\nnotin}{~{}\not\in{}~}
\newcommand{\wwedge}{~{}\wedge{}~}
\newcommand{\vvee}{~{}\vee{}~}

\newcommand{\cwedge}{\,{}\wedge{}\,}


%%Environments styles
\theoremstyle{plain}
\newtheorem*{thm*}{Theorem}
\newtheorem*{exmp*}{Example}
\newtheorem*{counterexmp*}{Counterexample}

\newtheoremstyle{ourstyle}{}{}{\itshape}{}{\bfseries}{.}{ }{\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}
%\newtheoremstyle{ourstyle}{}{}{}{}{\bfseries}{.}{ }{\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}
\theoremstyle{ourstyle}

\newcounter{ctdef}
\newcounter{ctlem}
\newcounter{ctprop}

\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}

% \newtheorem{theorem}{Theorem}
\newtheorem{definition}[ctdef]{Definition}
\newtheorem{lemma}[ctlem]{Lemma}
\newtheorem{property}[ctprop]{Property}
\newtheorem{corollary}[theorem]{Corollary}

%low-level lemma environment
\newtheoremstyle{llemstyle}{}{}{\itshape}{}{\bfseries}{.}{ }{\thmname{#1}~\thmnumber{\thectprop.#2}\thmnote{ (#3)}}
%\newtheoremstyle{ourstyle}{}{}{}{}{\bfseries}{.}{ }{\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}
\theoremstyle{llemstyle}

\newcounter{ctllem}
\newtheorem{llemma}[ctllem]{Lemma}

%\newtheorem*{problem_formu}{Problem Formulation}
%\newenvironment{problem_formulation}
%{\begin{mdframed}\begin{problem_formu}}
		%		{\end{problem_formu}\end{mdframed}}

\newtheoremstyle{exmpstyle}{}{}{}{}{\bfseries}{.}{ }{\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}
\theoremstyle{exmpstyle}

% \newtheorem{example}[theorem]{Example}
\newtheorem{counterexample}[theorem]{Counterexample}

\newtheoremstyle{rmkstyle}{}{}{}{}{\bfseries}{.}{ }{\thmname{#1}\thmnote{ (#3)}}
\theoremstyle{rmkstyle}

%\newtheorem{remark}[theorem]{Remark}
\newtheorem{remark}{Remark}

%\renewcommand{\qedsymbol}{$\blacksquare$}

%%\newtheorem{definition}{Definition}
%%\newtheorem{theorem}{Theorem}
%%\newtheorem{remark}{Remark}
%
%\newtheorem{thm}{Theorem}%[section]
%\newtheorem{lemma}[thm]{Lemma}
%\newtheorem{proposition}[thm]{Proposition}
%\newtheorem{corollary}{Corollary}
%\newtheorem{conj}{Conjecture}%[section]
%
%\theoremstyle{definition}
%\newtheorem{definition}{Definition}%[section]
%\newtheorem{example}{Example}%[section]
%\newtheorem{remark}{Remark}

%for qedT mark compatible within displaymath
\def\triangleforqed{\hbox{$\lhd$}}
\makeatletter
\DeclareRobustCommand{\qedT}{%
	\ifmmode
	\eqno \def\@badmath{$$}%$$
	\let\eqno\relax \let\leqno\relax \let\veqno\relax
	\hbox{\triangleforqed}%
	\else
	\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
	\quad\hbox{\triangleforqed}%
	\fi
}
\makeatother


%%% experiments
\newcommand{\best}[1]{{\textbf{#1}}}
\newcommand{\similar}[1]{{\underline{#1}}}


\newcommand{\aref}[1]{{Appx.~\ref{#1}}}

==> sections/dataset.tex <==
% !TEX root = ../main.tex
%
\section{Benchmark}\label{sec:benchmark}

This section describes our \emph{benchmark dataset for service regulation rules} ({\datasetname}, for short). This dataset is primarily used for
\begin{enumerate*}[label=(\roman*)]
	\item extracting key observations guiding the design of {\langname} as demonstrated in \cref{sec:language};
	\item fine-tuning {\gptname} to automate the modeling process in {\langname}; and
	\item evaluating future cross-domain models geared toward intelligent service regulation.
\end{enumerate*}
{\datasetname} is open-sourced via Hugging Face at \url{https://huggingface.co/datasets/Xfgll/SRR-Eval}.

The roadmap of constructing {\datasetname} is as follows: Albeit with numerous existing LLM datasets for testing general model understanding abilities, we need to \emph{create a dedicated dataset} for training and evaluating the model's understanding of regulation rules (written in natural language) and it's effectiveness to compile these rules into the {\langname} language. To this end, we start by \emph{collecting real-world regulation rules} with manually annotated {\langname} forms, which is, however, only possible for a few service regulation domains due to copyright and/or legal reasons. For instance, the ISO (International Organization for Standardization) standards encoding plenty of regulation rules are not freely distributed to the general public; financial services involving trade secrets typically do not allow direct access to their regulation rules. Therefore, we diversify our benchmark by \emph{generating quasi regulation rules} and their corresponding {\langname} forms leveraging state-of-the-art LLMs. Nonetheless, the so-obtained quasi rules may exhibit semantic contradictions against common sense and/or poor diversity in syntactic patterns, and hence we devise a method that combines conditional generation with manual screening to \emph{prune out semantic contradictions} and \emph{enforce syntactic diversity}.

\begin{figure*}[t]
	\centering
	\includegraphics[width=1\linewidth]{dataset}
	\caption{Overview of the bilingual {\datasetnameNaked} dataset.  \enquote{EN} and \enquote{CN} indicate rules in English and Chinese, respectively; \enquote{Real} marks domains where we collect real-world rules and unmarked ones are those with LLM-generated quasi rules.}
	\label{fig:dataset}
\end{figure*}

Below, we first give an overview of the {\datasetname} dataset, then provide technical details of collecting, generating, and formatting rules in {\datasetname}, and finally present a quality assessment of the underlying manual annotation process.

\paragraph*{\bf Overview of {\datasetnameNaked}}
\Cref{fig:dataset} sketches a bird's-eye perspective of our multilingual {\datasetname} dataset. It consists of 10 domains with real-world regulation rules (50 rules for each domain) and 40 domains with LLM-generated quasi rules (115 rules for each domain), thus amounting to \emph{50 domains with 5,100 rules} in total. All the involved domains are categorized into 4 fields of services covering industry and consumer services, technology and innovation, social regulation and governance, as well as environmental and resources. Every rule in {\datasetname} is structured and represented as a JSON object encoding its {\langname} form, which is obtained by either manual annotations (for real-world rules) or LLM-based generation (for quasi rules).

%In the previous discourse, we have fully defined a multimodal supervisory language applicable to a range of domains. The pertinent issue now is how to translate supervisory rules written in natural language into this formalized language. The usual approach is to train experts familiar with the supervisory language to dissect, translate, and compile specific rules. However, this manual method becomes impractical considering the vast number of rules in the real world and the continual emergence of new domains with additional rules. The natural language pre-trained large models possess text comprehension capabilities comparable to humans. Therefore, in this paper, we consider a natural language rule compiler based on large language models, named ParseGPT, which can automatically complete the compilation of specific natural language rules into a formalized supervisory language.

%In the real world, many domains are constrained or supervised by corresponding regulatory rules. Influenced by language types and expert expression habits, the same rule can have many different natural language expressions, even if the specific content to be regulated is the same. Therefore, automatically transforming language rules expressed in different ways into our designed unified supervisory language has become a new open problem that urgently needs to be addressed.
%%
%In the existing LLM benchmark datasets, there are already many datasets for testing model understanding abilities or performing common Q\&A tasks. However, due to the specificity of our task (testing the model's understanding of rule language) and its uniqueness (the tasks to be completed are not common types like choosing, summarizing, or text generation) the existing benchmark datasets do not fit well with our needs, namely to test the model's understanding of natural language rules and its compilation effectiveness. To solve this problem, we have designed a benchmark dataset FRR-Eval (Formalize Regulatory Rules).
%%
%In short, we have sourced regulatory rules of ten domains from open legal documents, public treaties of various companies, and free ISO standards, and processed each rule into the expression form of the supervisory language. Many domains, due to copyright and legal reasons, cannot directly open their data. In view of this, we will consider using the state-of-the-art large language model GPT-4 combined with manual supervision to generate quasi-regulatory rules and their corresponding language forms for forty popular domains.

\subsection{Dataset Construction}\label{subsec:dataset-construction}

\paragraph*{\it Collection}
We employ the following principles when collecting real-world regulation rules:
\begin{itemize}
  \item Ensure significant \emph{heterogeneity} between different domains to better test the model's ability to understand rules in various domain contexts.
  \item Seek out \emph{multilingual} rule data to assess the model's adaptability to rules in multiple languages.
  \item Ensure that the collected data is free, public, and available for download and editing.
\end{itemize}
%
In line with these principles, we have collected a total of 500 real-world rules evenly distributed across 10 regulation domains (see \cref{fig:dataset}), as well as their manually annotated {\langname} forms. These real-world rules will later be used to \emph{validate} the performance of our fine-tuned {\gptname}.
%five real datasets each in Chinese and English environments. The basic information of these ten datasets is shown in Fig.6, labeled as (Test). The Chinese datasets are sourced from municipal management regulations, public legal documents, and corporate public documents. The English datasets are derived from European Union laws (Eur-lex).

\paragraph*{\it Generation}
%Despite the abundance of regulatory rules in the real world, many domain-specific rules cannot be used as public datasets. For instance, the majority of current standards in ISO documents are not freely accessible; similarly, some domains involving trade secrets do not allow direct access to their regulatory rules. In light of this, 
We use GPT-4~\cite{openai2024gpt4} to generate quasi regulation rules covering 40 additional domains (cf.\ \cref{fig:dataset}) and their corresponding {\langname} forms. These quasi rules can be used either to \emph{train and test} cross-domain models like deep neural networks or, as in our case, to fine-tune existing LLMs. As an example, a quasi rule generated by GPT-4 for the domain of food safety may read as follows:
\begin{equation}\label{eq:quasi-rule-effective}
\begin{aligned}
	&\rulefont{Milk~cannot~be~sold~at~the~original~price} \\[-1mm]
	&\rulefont{within~\nblue{24}~hours~\green{before}~expiration.}
\end{aligned}\tag{R1}
\end{equation}%
Although Rule \cref{eq:quasi-rule-effective} deviates from its real-world counterpart, which may require a time window of $\rulefont{\nblue{12}~hours}$ instead of $\rulefont{\nblue{24}}$, it is considered to be \emph{effective} for training and testing the general ability to encode regulation rules in {\langname}. In contrast, the quasi rule
\begin{equation}\label{eq:quasi-rule-ineffective}
\begin{aligned}
	&\rulefont{Milk~cannot~be~sold~at~the~original~price} \\[-1mm]
	&\rulefont{within~\nblue{24}~hours~\maroon{after}~expiration.}
\end{aligned}\tag{R2}
\end{equation}%
is deemed \emph{ineffective} since it exhibits a \emph{semantic contradiction against common sense} and thus shall be excluded from the dataset. Such ineffective quasi rules are pruned out by means of a manual screening process, thereby yielding 50 effective quasi rules for each of the 40 domains.

%thereby obtaining more effective quasi-regulatory rules. Here, 'effective' means these rules closely resemble real-world regulations in form, utilizing complex natural language expressions and adapting the rule's phrasing according to the domain context. 'quasi-rules' refer to the fact that these regulatory rules do not actually exist and may contradict the real world. These contradictions are typically inherent to the rules themselves, rather than being contradictions of common sense, here is an example.

We further observe that the LLM-generated quasi rules often exhibit \emph{poor diversity in syntactic patterns}: For instance, a typical quasi rule in the domain of big data reads as follows:
\begin{equation}\label{eq:quasi-rule-poor-diversity}
	\begin{aligned}
		&\rulefont{The~collected~information~should~include~user~behavior} \\[-1mm]
		&\rulefont{data,~user~preference~data,~or~user~transaction~data.}
	\end{aligned}\tag{R3}
\end{equation}%
The {\langname} form of this quasi rule is
\begin{align*}
	\should \left( \event_{\textcolor{NavyBlue}{11}} \vee \event_{\textcolor{NavyBlue}{12}} \vee \event_{\textcolor{NavyBlue}{13}} \right)\quad \text{with}\\[-1.5\baselineskip]
\end{align*}%
\begin{align*}
	&\event_{\textcolor{NavyBlue}{11}} = \rulefont{The~collected~information~include~user~behavior~data.} \\[-1mm]
	&\event_{\textcolor{NavyBlue}{12}} = \rulefont{The~collected~information~include~user~preference~data.} \\[-1mm]
	&\event_{\textcolor{NavyBlue}{13}} = \rulefont{The~collected~information~include~user~transaction~data.}
\end{align*}%
where all the basic events $\event_{\textcolor{NavyBlue}{11}}$, $\event_{\textcolor{NavyBlue}{12}}$, and $\event_{\textcolor{NavyBlue}{13}}$ are of the same syntactic pattern, i.e., $\obj~\act~\obj$. 
The LLM-generated quasi rules of the form \cref{eq:quasi-rule-poor-diversity} are appropriate to train the model's ability to deconstruct original rules and extract the underlying logical relation between basic events. However, due to the poor diversity in syntactic patterns, they are \emph{insufficient} to train the model's ability to classify basic events into specific syntactic categories (cf.\ the bottom-level grammar of {\langname} in \cref{subsec:syntax}).

To enforce syntactic diversity, we use GPT-4 to generate 65 additional quasi rules for each of the 40 domains. These rules do not feature complex logical relations; rather, they are single-event rules covering all event patterns in {\langname}. For example, to match the pattern $\obj\mydot\attr~\diamond~\val$ in the domain of taxi services, GPT-4 generates	\begin{align}\label{eq:quasi-rule-single-event}
	\rulefont{The~response~delay~of~orders~shall~not~exceed~10mins.}\tag{R4}
\end{align}%

%\definecolor{111}{HTML}{2E75B6}
%
%\begin{tcolorbox}[attach title to upper,after title={:\ },enhanced,
%    colback=white,
%    opacityframe=0.4,
%    colframe=green!40!black]{\textbf{Real-World Rules:}}
%Milk cannot be sold at the original price within \textcolor{111}{12} hours \textcolor{red!60!green}{before} expiration.
%\end{tcolorbox}
%
%\begin{tcolorbox}[
%    enhanced,
%    overlay={
%        \node[draw=red!13!green!34!blue, rounded corners, fill=white, anchor=center, xshift=1.5cm,fill = red!6!green!14!blue!26!white] at (segmentation.west) {Evaluation};
%    },
%    colback=white,
%    opacityframe=0.5,
%    colframe=red!13!green!34!blue
%]
%\hspace*{-3mm}
%\begin{tabular}{p{7.5cm}m{0.5cm}}
%    \textbf{Generated Rules \#1:} Milk cannot be sold at the original price within \textcolor{111}{24} hours \textcolor{red!60!green}{before} expiration. & \color{ForestGreen}\ding{51} \\
%    \textbf{Generated Rules \#2:}  Milk cannot be sold at the original price \textcolor{111}{24} hours \textcolor{red!60!green}{after} expiration. & \color{Maroon}\ding{55} \\
%  \end{tabular}
%
%\tcblower
%
%The time constraint of Rule \#1 contradicts the actual rule but is considered an \textcolor{ForestGreen}{effective} quasi-rule.
%\vspace{2mm}
%
%The causal logic of Rule \#2 contradicts the actual rule and is considered an \textcolor{Maroon}{ineffective} quasi-rule.
%
%\end{tcolorbox}
%
%Above are two examples of contradictions. The first type of rule is reasonable. The contradiction arises because the generative model has not encountered real-world rules. The second type of contradiction violates logical relationships (such as milk not being sellable immediately upon expiration), making such rules unsuitable for downstream tasks.
%
%
%To obtain such valuable quasi-rules, the large language model GPT-4 is an excellent choice. Firstly, GPT-4 is currently the state-of-the-art model with the strongest comprehensive understanding and generative capabilities. Secondly, large language models possess strong generalization abilities, thereby enabling the generation of the "effective quasi-rules" we require. However, even GPT-4 can sometimes produce logically disorganized rule examples. To further improve the quality of generated rules, we designed a method combining conditional generation with manual screening.
%
%In the selected 40 domains, as shown in Fig.6, we generated two types of datasets with different purposes. The first type of dataset includes the original text of rules within a domain, a list of basic events extracted from these rules, and their logical relationships.The second type of dataset comprises various basic events from each domain and their corresponding syntactic types. The basic events in this dataset are not the same as those split from the first dataset, which relates to the different design objectives of the two datasets. The first dataset is intended to train the model's ability to deconstruct original rules and extract logical relationships, while the second is aimed at training the model's ability to classify given basic events into specific syntactic categories. The rationale behind this design will be discussed in Section 4.
%
%
%\definecolor{222}{HTML}{ED7D31}
%\definecolor{333}{HTML}{A2175F}
%\definecolor{444}{HTML}{385723}
%\definecolor{555}{HTML}{7C7C7C}
%\definecolor{666}{HTML}{176D55}
%
%\begin{tcolorbox}[enhanced,
%    colback=white,
%    opacityframe=0.4,
%    colframe=green!40!black,breakable,
%    attach boxed title to top left={yshift=-2mm,xshift=3mm},title=Type\#1  ,
%    colbacktitle=green!50!black,]
%{
%\textcolor{333}{[}
%
%\textcolor{555}{...}
%
%\textcolor{444}{\{}
%
%\hspace{5mm}\textbf{\textcolor{222}{"Original Rule"}\textcolor{555}{:}} \textcolor{666}{"The collected big data information should include user} \textcolor{666}{behavior data, user pref-}\textcolor{666}{erence data, or user transaction data."} \textcolor{555}{,}
%
%\hspace{5mm}\textbf{\textcolor{222}{"Basic Rules"}\textcolor{555}{:}} \textcolor{333}{[}
%
%\hspace{10mm}\textcolor{666}{"The collected big data information
%should include user behavior data"}\textcolor{555}{,}
%
%\hspace{10mm}\textcolor{666}{"The collected big data information
%should include user preference data"}\textcolor{555}{,}
%
%\hspace{10mm}\textcolor{666}{"The collected big data information
%should include user transaction data"}
%
%\hspace{5mm}\textcolor{333}{]} \textcolor{555}{,}
%
%\hspace{5mm}\textbf{\textcolor{222}{"Logical Relationship"}\textcolor{555}{:}} \textcolor{666}{"A\textbar{}B\textbar{}C"}
%
%\textcolor{444}{\}}\textcolor{555}{,}
%
%\textcolor{555}{...}
%
%\textcolor{333}{]}
%
%}
%
%\end{tcolorbox}
%
%\begin{tcolorbox}[enhanced,
%    colback=white,
%    opacityframe=0.5,
%    colframe=red!13!green!34!blue,breakable,
%    attach boxed title to top left={yshift=-2mm,xshift=3mm},title=Type\#2,
%    colbacktitle=red!13!green!34!blue,]
%{
%\textcolor{333}{[}
%
%\textcolor{555}{...}
%
%\textcolor{444}{\{}
%
%\hspace{5mm}\textbf{\textcolor{222}{"Basic Rule"}\textcolor{555}{:}}\textcolor{666}{"Collected personal
%information can only be stored for less than
%24 hours."}\textcolor{555}{,}
%
%\hspace{5mm}\textbf{\textcolor{222}{"Syntactic Type"}\textcolor{555}{:}}\textcolor{666}{"object attribute compare
%value"}
%
%\textcolor{444}{\}}\textcolor{555}{,}
%
%\textcolor{555}{...}
%
%\textcolor{333}{]}
%
%
%}
%\end{tcolorbox}
%
%Above is a simple example of these two types of datasets. In subsequent experiments, we will use real data as the validation set and generated data as the training and testing sets. 

\paragraph*{\it Formatting}
Our {\datasetname} dataset is represented as a JSON array. Every rule in the dataset is structured and represented as a JSON object in the array encoding its {\langname} form, which is obtained by either manual annotations (for real-world rules, used for validation) or LLM-based generation (for quasi rules, used for training and testing).

A real-world rule in the \emph{validation set} is encoded as a JSON object with the following key-value pairs:
\begin{itemize}
\item \jstring{original rule}: string(rule), 
\item  \jstring{basic events}: list[string(event)], 
\item  \jstring{logical relation}: string(symbolic representation),
\item  \jstring{syntactic patterns}: list[string(pattern)].
\end{itemize}
Here, the list of basic events and the list of syntactic patterns are of the same length; the logical relation is captured by a string, e.g., \jstring{A \& B \& (C $\vert$ D)} for encoding $A \land B \land (C \lor D)$, where $A$, $B$, $C$, and $D$ correspond to the first, second, third, and fourth basic event in the list, respectively.
%These logical strings are all in their simplest form. A composite rule is typically formed by a combination of basic events, following the definition: the smallest detectable unit in a rule. For example, the urban management rule "Manhole covers used for more than three years need to be replaced promptly" contains two detectable units and should be split into "Manhole covers used for more than three years" and "Manhole covers need to be replaced promptly", connected by "$\land $". Under the smallest detectable unit constraint, each rule has only one way to be split.

The quasi rules in the \emph{training and testing set} are encoded as JSON objects of two distinct forms. The first form encodes composite rules like \cref{eq:quasi-rule-poor-diversity} for training the ability to deconstruct original rules and extract the logical relation between basic events; it consists of three key-value pairs: 
\begin{itemize}
\item \jstring{original rule}: string(rule), 
\item  \jstring{basic events}: list[string(event)], 
\item  \jstring{logical relation}: string(symbolic representation).
\end{itemize}
We guide GPT-4 to generate these composite rules by specifying a variety of logical relations. Such guidance remedies the imbalance between logical connectives $\land$ and $\lor$.
The second JSON form encodes single-event rules like \cref{eq:quasi-rule-single-event} for training the ability to classify basic events into the given set of syntactic categories; it consists of two key-value pairs: 
 \begin{itemize}
\item  \jstring{basic events}: list[string(event)], 
\item  \jstring{syntactic patterns}: list[string(pattern)].
\end{itemize}
Akin to the first form, we can improve the syntactic diversity by enforcing syntactic patterns when generating the rules.
%Similar to the logical relationship, we start from the syntactic type to generate corresponding basic events that match the syntax, also to prevent data imbalance issues.

\subsection{Quality Assessment}\label{subsec:quality-assess}

To ensure the quality of manual annotations used for obtaining the {\langname} forms of real-world regulation rules, we provide training to volunteers on the task of annotation. We offer a concise tutorial and provide a representative set of example annotations as references. 
%labeled example rules to provide clear explanations for annotation requirements. 
For the annotation process, the rules of each domain are annotated by three volunteers independently. If the annotated {\langname} forms are syntactically consistent among the volunteers, the corresponding form is taken as the final result; Otherwise, the principle of \enquote{majority rules} is adopted.

We employ \emph{Fleiss' kappa}~\cite{fleiss1971measuring} -- a statistical measure used to evaluate the reliability and agreement among multiple annotators when %categorizing or 
classifying data into multiple categories. For each of the 10 regulation domains with real-world rules, the corresponding value of Fleiss' kappa is calculated as
\begin{align*}
	     \kappa \eeq \frac{P_o - P_e}{1 - P_e}~,
\end{align*}%
where $P_o$ is the \emph{observed agreement proportion} among annotators and $P_e$ is the \emph{expected agreement proportion}. Fleiss' kappa thus allows us to quantify the level of agreement beyond what would be expected by chance alone, thus providing valuable insights into the level of agreement among the annotators. For instance, the values of Fleiss' kappa for the domain of forest resource management and that of urban management are 0.845 and 0.864, respectively. These results indicate that our annotation consistency is at an \emph{almost perfect} agreement level ($0.81 \leq \kappa \leq 0.99$) as per \cite{landis1977measurement}.

% 城管逻辑关系标注：0.8641008914981517  EUR：0.8452331820057777

